Calibration Strategies for Robust Causal Estimation: Theoretical and Empirical Insights on Propensity Score-Based Estimators

The partitioning of data for estimation and calibration critically impacts the performance of propensity score based estimators like inverse probability weighting (IPW) and double/debiased machine learning (DML) frameworks. We extend recent advances in calibration techniques for propensity score estimation, improving the robustness of propensity scores in challenging settings such as limited overlap, small sample sizes, or unbalanced data. Our contributions are twofold: First, we provide a theoretical analysis of the properties of calibrated estimators in the context of DML. To this end, we refine existing calibration frameworks for propensity score models, with a particular emphasis on the role of sample-splitting schemes in ensuring valid causal inference. Second, through extensive simulations, we show that calibration reduces variance of inverse-based propensity score estimators while also mitigating bias in IPW, even in small-sample regimes. Notably, calibration improves stability for flexible learners (e.g., gradient boosting) while preserving the doubly robust properties of DML. A key insight is that, even when methods perform well without calibration, incorporating a calibration step does not degrade performance, provided that an appropriate sample-splitting approach is chosen.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> paper/sections/simulation/desirable_properties.tex <==
\subsection{Desirable Properties}
\begin{wrapfigure}{!r}{0.55\textwidth} 
\centering 
\includegraphics[width=0.53\textwidth]{paper/figures/figures_drug/paper_cov_balance/n_obs_02000_dim_x_003_clip_0.01_R2d_0.00_overlap_0.01_share_treated_0.00.pdf}
    \fbox{%
        \scriptsize
        \begin{tabular}{@{}l@{\hspace{1em}}llllll}
            % First Row
            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cbblack, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cbblack, circle, line width=0.8pt, fill=cbblack, minimum size=2pt] at (1em,0) {};
            \end{tikzpicture}} & Optweight &
            
            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cbdarkblue, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cbdarkblue, diamond, line width=0.8pt, fill=cbdarkblue, minimum size=2pt] at (1em,0) {};
            \end{tikzpicture}} & EBAL &

            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \node[color=cbgreen2] at (2em,0) {\Large$\times$};
            \end{tikzpicture}} & Alg-1-uncalib \\
            
            % Second Row
            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cbbrown, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cbbrown, regular polygon, regular polygon sides=3, fill=cbbrown, line width=0.8pt, minimum size=2pt] at (1em,0) {};
            \end{tikzpicture}} & IPT &

            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cbgrey, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cbgrey, regular polygon, regular polygon sides=3, shape border rotate=270, fill=cbgrey,line width=0.8pt, minimum size=2pt] at (1em,0) {};
            \end{tikzpicture}} & GLM &

            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cbmagenta, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cbmagenta, regular polygon, regular polygon sides=3, shape border rotate=180, line width=0.8pt,fill=cbmagenta, minimum size=0.5pt] at (1em,0) {};
            \end{tikzpicture}} & Alg-5-full-sample \\
            
            % Third Row
            \raisebox{0.5ex}{\begin{tikzpicture}[baseline=-0.5ex]
                \draw[color=cborange, line width=1.5pt] (0,0) -- (2em,0);
                \node[draw=cborange, regular polygon, regular polygon sides=5, shape border rotate=0, fill=cborange,line width=0.8pt, minimum size=2pt] at (1em,0) {};
            \end{tikzpicture}} & GLM \\
            
        \end{tabular}%
    }
\caption{SMD across covariates for DGP 2. Dashed line indicates \(|\text{SMD}| = 0.1\).}
\label{fig:cov_balance_plot}
\end{wrapfigure}
Modern causal inference methods using weighting estimators address two core challenges: (1) achieving covariate balance, where the weighted covariate distributions satisfy \(\mathbb{E}[w \mathbf{X} \mid D=1] = \mathbb{E}[w \mathbf{X} \mid D=0]\) for treatment \(D \in \{0,1\}\) and covariates \(\mathbf{X}\), and (2) ensuring normalization \(\sum_{i: D_i=1} w_i = 1\) and \(\sum_{i: D_i=0} w_i = 1\) to stabilize weights \citep{busso2014normalizedweights}. Covariate balance is quantified via standardized mean differences (SMD): 
\[
\text{SMD}_k = \frac{\bar{X}_{k,D=1}^w - \bar{X}_{k,D=0}^w}{\sqrt{(s_{k,D=1}^w)^2 + (s_{k,D=0}^w)^2}/2},
\]
where \( \bar{X}_{k,D}^w \) and \( s_{k,D}^w \), with \(D \in \{0,1\}\), are the weighted means and standard deviations of \( X_k \) in the treated and control groups, respectively.
The SMD expresses an imbalance in standard deviation units, with \(|\text{SMD}_k| < 0.1\) indicating an adequate balance \citep{austin2015covbalance}. Figure~\ref{fig:cov_balance_plot} demonstrates SMD reduction across methods. Entropy balancing (EBAL) minimizes KL/ Rényi divergence from uniform weights \(q_i = 1/n\) under balance constraints \(\sum_{i: D_i=0} w_i \phi(\mathbf{X}_i) = \frac{1}{n_1} \sum_{i: D_i=1} \phi(\mathbf{X}_i)\) \citep{hainmueller2012ebalatt}. OptimWeight solves \(\min_w\) \(\sum_{i: D_i=0} (w_i - 1/n_0)^2\) with \(\ell_\infty\)-norm balance constraints \(\| \frac{1}{n_1} \sum_{i: D_i=1} \mathbf{X}_i - \sum_{i: D_i=0} w_i \mathbf{X}_i \|_\infty\) \(\leq \delta\) \citep{zubizarreta2015optweight}. Covariate balancing propensity score (CBPS) estimates the propensity score \(m(\mathbf{X}_i;\beta) = \text{expit}(\mathbf{X}_i^T \beta)\) via GMM, combining score equations \(\sum_{i=1}^n [D_i - m(\mathbf{X}_i;\beta)] \mathbf{X}_i = 0\) with balancing moments \cite{imai2014cbps}. Inverse probability tilting (IPT) solves dual-moment conditions for normalization \(\sum D_i/m(\mathbf{X}_i; \theta) = n\) and balance \(\sum D_i \mathbf{X}_i/m(\mathbf{X}_i;\theta)\) \(= \sum (1-D_i) \mathbf{X}_i/(1 - m(\mathbf{X}_i;\theta))\) \citep{graham2012ipt}. GLM uses \(m(\mathbf{X}_i) = \text{expit}(\mathbf{X}_i^T \hat{\beta}_\text{MLE})\) with normalized IPW weights. 
To ensure a fair comparison, only first-order moments were rebalanced in the setup of the outcome equation for the \texttt{weightit} approaches. 
Similarly, Alg-\ref{main-alg:dml2:calibration}-cf and Alg-\ref{main-alg:dml2:calibration_all}-full-sample used a linear outcome function without further fine-tuning, as excessive fine-tuning could bias the comparison. This means the outcome equation is misspecified for all methods. Figure~\ref{fig:cov_balance_plot} shows that methods from the R package \texttt{weightit} \citep{greifer2025weightit} (EBAL, OptWeight, CBPS, GLM, IPT) as well as the full-sample calibrated IRM model achieve covariate balance, unlike the unadjasted IRM model. Table~\ref{tab:weightit_comp} compares performance metrics and normalization. 

\begin{table}[htb]
\begin{center}
\captionsetup{justification=centering}
\caption{Comparison under covariate balance}
\label{tab:weightit_comp}
    \begin{footnotesize}
    \begin{singlespace}
        \scalebox{0.9}{
\centering
\begin{tabular}{lllrrrrrrrr}
\toprule
Method &  & m & Coverage & CI Length & Norm $D=1$ & Norm $D=0$ & RMSE & Std. dev. & MAE \\
\midrule
Alg-3-cf & isotonic & Logit & 0.960 & 0.413 & 0.996 & 0.987 & 0.098 & 0.097 & 0.077 \\
Alg-3-cf & isotonic & RF & 0.960 & 0.389 & 0.997 & 0.994 & 0.096 & 0.094 & 0.075 \\
Alg-3-cf & platt & Logit & 0.960 & 0.388 & 1.003 & 0.984 & 0.094 & 0.093 & 0.075 \\
Alg-3-cf & platt & RF & 0.940 & 0.358 & 0.984 & 0.961 & 0.092 & 0.091 & 0.072 \\
Alg-5-full-sample & isotonic & Logit & 0.970 & 0.404 & 0.999 & 0.998 & 0.097 & 0.095 & 0.077 \\
Alg-5-full-sample & isotonic & RF & 0.940 & 0.386 & 1.000 & 1.000 & 0.095 & 0.094 & 0.075 \\
Alg-5-full-sample & platt & Logit & 0.960 & 0.397 & 1.003 & 0.996 & 0.094 & 0.093 & 0.075 \\
Alg-5-full-sample & platt & RF & 0.950 & 0.373 & 0.998 & 0.988 & 0.094 & 0.093 & 0.074 \\
Cbps & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.074 \\
Ebal & weighted & - & 0.950 & 0.376 & 1.000 & 1.000 & 0.094 & 0.093 & 0.074 \\
Glm & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.075 \\
Ipt & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.075 \\
Optweight & weighted & - & 0.960 & 0.376 & 1.000 & 1.000 & 0.093 & 0.092 & 0.074 \\
\bottomrule
\end{tabular}
}
\caption*{\scriptsize DGP 2: n = 2000, p = 3, overlap = 0.5, Clip = 1e-12 g = Linear}
    \end{singlespace}
    \end{footnotesize}
    		\end{center}
\end{table}
\vspace{-2em}
All \texttt{weightit} methods enforce exact normalization via $\mathbb{E}[D/m(\mathbf{X})] = 1$ and $\mathbb{E}[(1-D)/(1-m(\mathbf{X}))] = 1$ (columns 'Norm D = 1' and 'Norm D = 0'), ensuring weight stability. Full-sample calibration achieves higher levels of normalization compared to their cross-fitted counterparts. However, the remaining small deviations from optimally normalized weights do not deteriorate performance, as seen in Table~\ref{tab:weightit_comp}.

==> paper/sections/simulation/detailed_dgps.tex <==
\begin{table}[H]
\begin{center}
\begin{footnotesize}
\begin{singlespace}
\caption{Overview of the DGPs}
    \begin{tabular}{llll}
        \toprule
        \textbf{DGP} & \textbf{Covariates} & \textbf{Description of \( D \mid X \)} & \textbf{Description of \( g_0(D, X) \)} \\
        \hline
        \multirow{4}{*}{1} & \multirow{4}{3cm}{$X_i \sim N(0, \Sigma)$ with $\Sigma_{kj} = (0.5)^{|j-k|}$} & \multirow{4}{4cm}{Sigmoid function combined with Uniform indicator. $D$ is exogenous conditional on $X$.} & \multirow{4}{5cm}{Heterogeneous treatment effect, linear with simple interaction, $\epsilon_i \overset{\text{iid}}{\sim} \mathcal{N}(0,1)$} \\
        & & & \\
        & & & \\
        & & & \\
        \hline
        \multirow{4}{*}{2} & \multirow{4}{3cm}{$X_1 \sim \text{Bin}(1, 0.5), X_2 \mid X_1 \sim \Gamma, X_3 \mid X_2 \sim \text{Beta}$} & \multirow{4}{4cm} {Highly nonlinear, tree-based via conditions, $D \sim \text{Bin}(1, m_0(X))$} & \multirow{4}{5cm}{Homogeneous treatment effect, Poisson with simple linear combination of covariates} \\
        & & & \\
        & & & \\
        & & & \\
        \hline
        \multirow{4}{*}{3} & \multirow{4}{3cm}{$X \sim \text{Unif}[-1,1]^4$} & \multirow{4}{4cm}{$\text{Expit}$ function combined with $D \sim \text{Bin}(1, m_0(X))$} & \multirow{4}{5cm}{Heterogeneous treatment effect, nonlinear transformations of the covariates, $\epsilon_i \overset{\text{iid}}{\sim} \mathcal{N}(0,1)$} \\
        & & & \\
        & & & \\
        & & & \\
        \hline
        \multirow{4}{*}{4} & \multirow{4}{3cm}{$X \sim \text{Unif}[0,1]^{20}$} & \multirow{4}{4cm}{Unbalanced and nonlinear $m_0(X) = \alpha \left(1+\beta_{2,4}(\min(X_1, X_2)) \right)$, $D \sim \text{Bin}(1, m_0(X))$} & \multirow{4}{5cm}{Heterogeneous treatment effect, scaled Friedman function for $g_0(X)$ and simple interaction of $D$ and $X$, $\epsilon_i \overset{\text{iid}}{\sim} \mathcal{N}(0,1)$} \\
        & & & \\
        & & & \\
        & & & \\
\bottomrule
\end{tabular}
    \caption*{A detailed description of DGP 2-4 is given in the Supplementary Material.}
    \end{singlespace}
    \end{footnotesize}
\end{center}
\end{table}
\vspace{-2.5em}


In our first DGP, data units were generated following \citet{belloni2017program}\footnote{This DGP is available at \hyperlink{https://docs.doubleml.org/stable/api/generated/doubleml.datasets.make_irm_data.html}{DoubleMLIRMData}.}.

DGP 2 is adapted from \citet{deshpande2023calibrated}. Three covariates are simulated: gender ($X_1$), age ($X_2$), and disease severity ($X_3$), while treatment ($D$) corresponds to the administration of a drug. The outcome $Y$ is the time taken for the recovery of a patient. In addition to the original setting, we introduced non-deterministic treatment assignments to ensure positivity. The function for the treatment assignment resembles the approach of tree-based models, favoring the IRM and PLR in combination with LGBM and random forest.

For a complicated nonlinear outcome regression, we implemented DGP 3 \citep{van2023causal}. The included transformations make it difficult for linear models as well as tree-based classifiers through the local linearity. Given the nonlinear and heterogeneous influence of the treatment on the outcome, we expect the IRM model to outperform the PLR. However, the treatment assignment itself can be modeled consistently, favoring the IPW.

The unbalanced treatment assignment DGP 4 follows \citet{ballinari2024calibrating} and is adapted from \citet{nie2020unbalanced}. Three settings of the share of treated \(\E[D]\) are tested: \(\E[D] \in \{0.05, 0.1, 0.2\}\). To address positivity violations, we tested three clipping thresholds for the propensity scores: \(1e-12\), \(0.01\), and \(0.1\). Given the majority non-treatment class, a lower threshold is sufficient to limit the contribution of a single observation.


\subsubsection*{DGP 1 IRM, Detailed Description}

\begin{align*}d_i &= 1\left\lbrace \frac{\exp(c_D X_i' \beta)}{1+\exp(c_D X_i' \beta)} > V_i \right\rbrace, & &V_i
\sim \mathcal{U}(0,1),\\y_i &= \theta D_i + c_Y X_i' \beta D_i + \zeta_i, & &\zeta_i \sim \mathcal{N}(0,1),
\end{align*} 
where $v_i \sim U(0,1)$, $\zeta_i \sim N(0,1)$, $V_i$ and $\zeta_i$ are independent, $p = \dim(X_i)$, the covariates $X_i \sim N(0,\Sigma)$ with $\Sigma_{kj} = (0.5)^{|j-k|}$.  $\beta$ is a $p \times 1$ vector with elements set as $\beta_{1,j} = (1/j)^2$ for $j = 1,...,p$.  $c_D$ and $c_Y$ are scalars given by
\begin{align*}c_Y = \sqrt{\frac{R_Y^2}{(1-R_Y^2) \beta' \Sigma \beta}}, \qquad c_D =
\sqrt{\frac{(\pi^2 /3) R_D^2}{(1-R_D^2) \beta' \Sigma \beta}}.
\end{align*}
that control the strength of the relationship between the controls, the outcome, and the treatment variable.
The underlying treatment effect is heterogeneous. Hence, to accurately model the interaction effects between treatment and covariates, the IRM should be considered. Simple propensity score weighting in the IPW, as well as the additive structural form assumptions for the treatment effect of the PLR, should be inconsistent for this DGP.


\subsubsection*{DGP 2 Drug Effectiveness, Detailed Description}

In our second DGP, data units were generated as follows:  
\begin{itemize}
    \item Gender indicator \(X_1\) and age \(X_2\) are simulated as:
\[ X_1 \sim \text{Bin}(0, 0.5), \quad
    X_2 \sim \Gamma(\kappa_{\text{age}}, \psi_{\text{age}}).
     \]
     The distribution of age is gender dependent:
    \[
    \kappa_{\text{age}} = \left( \frac{\mu_{\text{age}}}{\sigma_{\text{age}}} \right)^2, \quad
    \psi_{\text{age}} = \frac{\sigma_{\text{age}}^2}{\mu_{\text{age}}}, \text{ and}
    \]
    \[
    \mu_{\text{age}} = 
    \begin{cases} 
    49 & \text{if } X_1 = 1, \\ 
    51 & \text{if } X_1 = 0, 
    \end{cases} \quad 
    \sigma_{\text{age}} = 
    \begin{cases} 
    7 & \text{if } X_1 = 1, \\ 
    8 & \text{if } X_1 = 0.
    \end{cases}.
     \]


    \item Disease severity \(X_3\) is simulated based on age:
\[
    \mu_{\text{disease}} = \text{clip}\left( \frac{X_2 - 20}{20}, 0.1, 5 \right), \quad
    X_3 \sim \text{Beta}(\mu_{\text{disease}}, 2).
    \]
    
    \item Propensity scores are generated using linear predictors, incorporating adjustable levels of overlap through the parameter $\beta$:
\[
\text{coefficients} =     \left[
\begin{array}{l}
(-0.4, 0.2, 0.8), \\
(-0.4 + 2(1 - \beta), 0.2, 0.8), \\
(-0.4 + 2(1 - \beta), 0.3, 1), \\
(-0.4 + 2(1 - \beta), 0.1, 1.2), \\
(-0.4 + 2(1 - \beta), 0.1, 1.2)
\end{array}
    \right],
\]
\begin{align*}
\text{linear\_predictors} = \Big( & b_0 + b_1 \cdot \text{normalize}(X_2) + b_2 \cdot \text{normalize}(X_3) \\
& + \epsilon \mid (b_0, b_1, b_2) \in \text{coefficients} \Big), \\
& \epsilon \sim \mathcal{N}(0, 0.5).
\end{align*}
    Propensity scores are computed via logistic transformation:
\[
    \text{prop\_scores} = \left[ \frac{1}{1 + \exp(-\text{lp})} \mid \text{lp} \in \text{linear\_predictors} \right].
    \]
    
    \item Treatment assignment \(m_0\) is initialized with \(\text{prop\_scores}[0]\) and updated based on conditions:
\[
    \text{conditions} = 
    \begin{cases}
    ((X_1 = 0) \text{ and } (X_2 > 55) \text{ and } (X_3 \leq 0.55), \text{prop\_scores} [1]), \\ 
    ((X_1 = 1) \text{ and } (X_2 > 55) \text{ and } (X_3 \leq 0.55), \text{prop\_scores} [2]), \\
    ((X_1 = 0) \text{ and } (X_3 > 0.55), \text{prop\_scores} [3]), \\
    ((X_1 = 1) \text{ and } (X_3 > 0.55), \text{prop\_scores} [4]) 
    \end{cases}
\]    
\[
    \text{for } (\text{condition}, \text{score}) \in \text{conditions}: m_0[\text{condition}] = \text{score}[\text{condition}].
    \]
    Final treatment assignment \(D_i\) is:
\[
    D_i \sim \text{Bin}(1, m_0).
    \]
    \item The outcome \(Y_i\) is simulated as:
\[
    Y_{di} = \text{Pois}(2 + 0.5 X_1 + 0.03 X_2 + 2 X_3 - d), \qquad
    Y_i = D_i \cdot Y_{1i} + (1 - D_i) \cdot Y_{0i}.
    \]
\end{itemize}

This DGP captures complex relationships between gender, age, disease severity, and treatment assignment, providing a realistic framework for evaluating causal inference methods. The treatment assignments are highly nonlinear and resemble decision trees with underlying local linearities. \\


\subsubsection*{DGP 3 Nonlinear, Detailed Description}

For the nonlinear outcome regression, the detailed data generation process is as follows:

\begin{align*}
    &X \sim \text{Unif}[-1,1]^{4}, \quad D \vert X \sim \text{Bin}(1,p(X)),\quad Y \sim \text{Bin}(1, \mu(X,D))
\end{align*}
with the treatment assignment probability given by:
\begin{equation*}
p(X)=\text{expit}\{-0.25 - X_1 + 0.5X_2 - X_3 + 0.5X_4\}.
\end{equation*}

The outcome function is based on nonlinear transformations of the covariates, with added treatment effect interactions. 
\begin{align*}
    &\mu(X,D)=1.5 + 1.5  D + 2  D  |X_1|  |X_2| - 2.5  (1-D) |X_2| X_3 + 2.5  X_3\\
    & + 2.5  (1-D)  \sqrt{|X_4|} -1.5  D \cdot I(X_2 < 0.5) + 1.5  (1-D) I(X_4 < 0).
\end{align*}

The outcome is then generated by:
\begin{align*}
Y_d  \sim \text{N}(\mu(X,D), 1), \quad  Y = DY_1 + (1-D)Y_0.
\end{align*} \\


\subsubsection*{DGP 4 Unbalanced, Detailed Description} 

The unbalanced treatment assignment setting follows \citet{ballinari2024calibrating} and is adapted from \citet{nie2020unbalanced}.
\begin{align*}
    X_i &\sim \text{Unif}[0,1]^{20}, \quad D \vert X \sim \text{Bin}(1, p(X)), \quad \epsilon_i \overset{\text{iid}}{\sim} \mathcal{N}(0,1), \\
    Y &= b(X) + (D-0.5) (X_1 + X_2) + \epsilon_i.
\end{align*}

The baseline main effect is the scaled \citet{friedman1991multivariate} function:
\[
b(X_i) = \sin(\pi X_1 X_2) + 2(X_3-0.5)^2 + X_4 + 0.5X_5.
\]

For the propensity score, we follow \citet{Kunzel2019meta} and set:

\[
m_0(X) = \alpha \left(1+\beta_{2,4}(\min(X_1, X_2)) \right),
\]

where \(\beta_{2,4}(\cdot)\) is the beta cumulative distribution function with shape parameters 2 and 4. This unbalanced setting entails difficult nuisance components and an easy treatment effect function, favoring doubly robust causal models compared to IPW.

The share of treated is \(\E[D] = (31/21) \alpha\). Three settings of the share of treated \(\E[D]\) are tested: \(\E[D] \in \{0.05, 0.1, 0.2\}\). For unbalanced applications, several adjustments for ATE estimators exist to address positivity violations. The most commonly used method is clipping the propensity scores to preset levels. Throughout our simulations, we tested three different levels of clipping thresholds.

As \citet{imbens2004trim} points out, for the IPTW with \(n=4000\) observations, choosing a clipping cut-off at \(0.01\)\footnote{Given the majority non-treatment class, a lower threshold is sufficient.} limits the contribution of a single observation to \(0.025\). We also tested more severe clipping as employed in \citet{nie2020unbalanced}, with a clipping level at \(0.1\), and alternatively, without clipping \footnote{To ensure computational stability we set the threshold at \(1e-12\).}. Particularly, for the setting with only \(5\%\) treated, we expect that a clipping threshold of \(0.1\) introduces a strong bias.

\newpage

==> paper/sections/simulation/platt.tex <==
\subsection{Platt Scaling}

Platt scaling \citep{platt1999plattscale} leverages the robust calibration properties of log-loss. It applies logistic regression, expressed by the function
\begin{equation*} 
    g(m(x)) := \frac{1}{1 + \exp(A m(X) + B)},
\end{equation*}
to the scores produced by an estimator, using treatment assignment labels as targets for calibration, where $A < 0$ and $B$ are parameters. The parameters $A$ and $B$ are estimated using a maximum likelihood method on the same training set as the original classifier $m(X)$. To avoid overfitting, a held-out calibration set or cross-validation can be used. Platt also recommends clipping the outputs $d$ to target probabilities in the range
\begin{equation*}\label{eq:range}
  \left(
    \frac{1}{N_0 + 2},
    \frac{N_1 + 1}{N_1 + 2}
  \right),
\end{equation*}
where $N_0$ is the number of control units and $N_1$ is the number of treated units in the calibration set. This motivates the testing of additional clipping in small sample sizes, a setting where the parametric form assumption is especially appropriate.


==> paper/sections/simulation/simulation_drug_effect.tex <==
\textbf{DGP 2 Drug Effectiveness}

We simulate the covariates as
\begin{align*}
    X_1 \sim \text{Bin}(1,0.5) && X_2 \sim \text{Gamma}(\alpha=8, \beta=4) && X_3 \sim \text{Beta}(\alpha=3, \beta=1.5).
\end{align*}
The outcome is simulated as 
The following simulation is adapted from \cite{deshpande2023calibrated}. Three covariates are simulated: gender ($X_1$), age ($X_2$), and disease severity ($X_3$), while treatment ($D$) corresponds to the administration of a drug. The outcome $Y$ is the time taken for the recovery of a patient. The data is generated as follows:
\begin{align*}
& x_1 \sim \text{Bernoulli}(0.5), \quad x_2 \mid x_1 \sim \Gamma\left( \left( \frac{X_1}{\sigma_{X_1}} \right)^2, \frac{\sigma_{X_1}^2}{X_1} \right) \\ 
& x_3 \mid x_2 \sim B\left( \text{clip}\left( \frac{x_2 - 20}{20}, 0.1, 5 \right), 2 \right), \quad d_i \mid x_i \sim \text{Bernoulli}(m_0(x_i)), \\ 
& y_i = d_i \times y_1(x_i) + (1 - d_i) \times y_0(x_i) \end{align*}
Gender ($x_1$) is simulated as a binary variable indicating male ($x_1 = 1$) or female ($x_1 = 0$) with equal probability. Age ($x_2$) is drawn from a gamma distribution, with parameters depending on gender, where males tend to have a lower average age. Disease severity ($x_3$) is drawn from a Beta distribution, conditioned on age, indicating higher severity with increasing age.
In addition to the original setting, we introduced non-deterministic treatment assignments to ensure positivity. The ground truth ATE ($\theta_0$) equals -1. The function for the treatment assignment resembles the approach of tree-based models. A detailed description is given in Appendix \ref{sec:extradgp}. 

==> paper/sections/simulation/simulation_irm.tex <==
In our first DGP, data units were generated following \citet{belloni2017program}:
\begin{align*}d_i &= 1\left\lbrace \frac{\exp(c_D X_i' \beta)}{1+\exp(c_D X_i' \beta)} > V_i \right\rbrace, & &V_i
\sim \mathcal{U}(0,1),\\y_i &= \theta D_i + c_Y X_i' \beta D_i + \zeta_i, & &\zeta_i \sim \mathcal{N}(0,1),
\end{align*} 
where $v_i \sim U(0,1)$, $\zeta_i \sim N(0,1)$, $V_i$ and $\zeta_i$ are independent, $p = \dim(X_i)$, the covariates $X_i \sim N(0,\Sigma)$ with $\Sigma_{kj} = (0.5)^{|j-k|}$.  $\beta$ is a $p \times 1$ vector with elements set as $\beta_{1,j} = (1/j)^2$ for $j = 1,...,p$.  $c_D$ and $c_Y$ are scalars given by
\begin{align*}c_Y = \sqrt{\frac{R_Y^2}{(1-R_Y^2) \beta' \Sigma \beta}}, \qquad c_D =
\sqrt{\frac{(\pi^2 /3) R_D^2}{(1-R_D^2) \beta' \Sigma \beta}}.
\end{align*}
that control the strength of the relationship between the controls, the outcome, and the treatment variable.
The underlying treatment effect is heterogeneous. Hence, to accurately model the interaction effects between treatment and covariates, the IRM should be considered. Simple propensity score weighting in the IPW, as well as the additive structural form assumptions for the treatment effect of the PLR, should be inconsistent for this DGP.


==> paper/sections/simulation/simulation_nonlinear.tex <==
\subsection*{DGP 3 Nonlinear}

For a nonlinear outcome regression, we used a DGP from \cite{van2023causal}. The data is generated with covariates \(X \sim \text{Unif}[-1,1]^{4}\), treatment assignment \(D \sim \text{Bin}(1, p(X))\), and outcome \(Y \sim \text{Bin}(1, \mu(X, D))\). The treatment assignment probability is given by:
\[
p(X) = \text{expit}\{-0.25 - X_1 + 0.5X_2 - X_3 + 0.5X_4\}.
\]
We consider two different settings for the outcome function:
\begin{itemize}
    \item[] \textbf{Setting A:} Shared outcome function, independent of the treatment assignment.
\item[] \textbf{Setting B:} Separate outcome functions, dependent on whether treatment occurred.
\end{itemize}

Note that in both settings, we anticipate difficulties in modeling the outcome regression due to underlying nonlinearities and complex interactions. Given the nonlinear and heterogeneous influence of the treatment on the outcome, we expect the IRM model to outperform the PLR. However, the treatment assignment itself can be modeled consistently, favoring the IPW. In Setting B, there is a violation of the unconfoundedness assumption. Hence, we anticipate inconsistent ATE estimation for all causal models.



==> paper/sections/simulation/simulation_unbalanced.tex <==
\subsection*{DGP 4 Unbalanced}

The unbalanced treatment assignment setting follows \cite{ballinari2024calibrating} and is adapted from \cite{nie2020unbalanced}. Covariates are generated as \(X_i \sim \text{Unif}[0,1]^{20}\). Treatment assignment is \(D \sim \text{Bin}(1, p(X))\), and the outcome is generated by:
\[
y = b(X) + (d-0.5) (X_1 + X_2) + \epsilon_i,
\]
where \(\epsilon_i \sim \mathcal{N}(0,1)\). The propensity score is given by:
\[
p(X) = \alpha \left(1+\beta_{2,4}(\min(X_1, X_2)) \right),
\]
with \(\beta_{2,4}(\cdot)\) being the beta cumulative distribution function with shape parameters 2 and 4.

Three settings of the share of treated \(\E[D]\) are tested: \(\E[D] \in \{0.05, 0.1, 0.2\}\). To address positivity violations, we tested three trimming thresholds for the propensity scores: \(1e-12\), \(0.01\), and \(0.1\). Given the majority non-treatment class, a lower threshold is sufficient to limit the contribution of a single observation.



==> paper/sections/simulation/vennabers.tex <==
\subsection{Venn-Abers Calibration}

Venn-Abers predictors \citep{vovk2004calibration} generate multi-probabilistic outputs for each target class, ensuring, by construction, one valid probability distribution. For binary classification, \cite{vovk2014vennaberspredictors} proposed Venn-Abers calibration, which uses isotonic regression over imputations \( d \in D \) of the unseen outcome \( D_{l+1} \). Such that each test unit \( W_{l+1} \) undergoes two isotonic regressions for \( d_{l+1} = 0 \) and \( d_{l+1} = 1 \), preventing overfitting. 

Typically, Venn-Abers predictors are computationally intensive. To address this, Inductive Venn-Abers predictors (IVAP) \citep{lambrou2012ivap, nouretdinov2018ivap} are utilized. The training set is split into a \emph{proper training set} and a \emph{calibration set}. Let $\hat{m}:\mathbf{X}\to\mathbb{R}$ be the fitted propensity learner. The isotonic calibrators $\tilde{m}_0$ and $\tilde{m}_1$ are fitted for:
$$
\{(\hat{m}(x_{k+1}), d_{k+1}), \ldots, (\hat{m}(x_l), d_l), (\hat{m}(x), 0)\}
$$
and
$$
\{(\hat{m}(x_{k+1}), d_{k+1}), \ldots, (\hat{m}(x_l), d_l), (\hat{m}(x), 1)\},
$$
respectively. IVAP outputs $(p_0, p_1)$, where $p_0 := \tilde{m}_0(\hat{m}(x))$ and $p_1 := \tilde{m}_1(\hat{m}(x))$.\footnote{Implemented in \texttt{Python} package \texttt{venn-abers 1.4.1}.}

In the case of the square loss function, the single calibrated probability is obtained through the formula:
\begin{equation}\label{eq:square}
  p = p_1 + \frac{p_0^2}{2} - \frac{p_1^2}{2}.
\end{equation}
As \cite{vovk2014vennaberspredictors} point out, this can be rewritten as:

\[
  p = \bar{p} + (p_1 - p_0) \left(\frac{1}{2} - \bar{p}\right),
\]

where $\bar{p} := \frac{p_0 + p_1}{2}$. Thus, $p$ is a regularized version of $\bar{p}$ moving the prediction towards $\frac{1}{2}$. This characteristic is particularly advantageous in mitigating the risk of inflated weights during treatment effect estimation.


==> paper/sections/theory/PLM.tex <==
\subsection{Calibration in Partially Linear Regression Models}\label{ch:plm}

Consider the partially linear regression model as in \citet{Chernozhukov2018dml}. Let $D\in\{0,1\}$ be a binary treatment variable and $W=(Y,D,X)$, where
\begin{align}
    Y = \theta_0 D + g_0(X) + U, \;  \E[U|D,X] &= 0, &
    D = m_0(X) + V, \;  \E[V|X] &=0, \label{PLR}
\end{align}
with $\theta_0$ being the parameter of interest. Let
\begin{align*}
    \psi(W;\theta,\eta):= (Y - l(X) - \theta(D-m(X))(D-m(X))
\end{align*}
be the "partialling-out" score function, where $\eta=(l,m)$ denotes the nuisance functions for the outcome regression $l_0(X) = \mathbb{E}[Y|X]$ and propensity score $m_0(X)=\mathbb{E}[D|X]$.

\begin{assumption}[cf. Assumption 4.1 in \citet{Chernozhukov2018dml}]\label{assumption::plm}
Let $(\delta_N)_{n=1}^\infty$ and $(\Delta_N)_{n=1}^\infty$ be sequences of positive constants approaching 0 as before. Also, let $c, C$ and $q$ be fixed strictly positive constants such that $q > 4$, and let $K \geq 2$ be a fixed integer. Moreover, for any $\eta = (\eta_1, \eta_2)$, where $\eta_1$ and $\eta_2$ are functions mapping the support of $X$ to $\mathbb{R}$, denote $\|\eta\|_{p,q} = \|\eta_1\|_{p,q} \lor \|\eta_2\|_{p,q}$. For simplicity, assume that $N/K$ is an integer. For all probability laws $P\in\mathcal{P}$ for the triple $(Y,D,X)$, the following conditions hold: 
\begin{itemize}
    \item[(a)] Equations \eqref{PLR} hold
    \item[(b)] $\|Y\|_{P,q} + \|D\|_{P,q} \leq C$
    \item[(c)] $\|UV\|_{P,2}\ge c^2$ and $\E_P[V^2]\ge c$
    \item[(d)] $\|\mathbb{E}_P[U^2 \mid X]\|_{P,\infty} \le C$ and $\|\mathbb{E}_P[V^2 \mid X]\|_{P,\infty} \leq C$
    \item[(e)] Given a random subset $I$ of $[N]$ of size $n = N/K$, the nuisance parameter estimator $\hat{\eta}_0 = ((W_i)_{i\in I^c})$ obeys the following conditions for all $N \geq 1$. With $P$-probability no less than $1 - \Delta_N$,
    \begin{itemize}
        \item[(i)] $\|\hat{\eta}_0 - \eta_0\|_{P,q} \leq C$ and $\|\hat{\eta}_0 - \eta_0\|_{P,2} \leq \delta_N$
        \item[(ii)] $\|\hat{m}_0 - m_0\|_{P,2} \times \Big(\|\hat{m}_0 - m_0\|_{P,2} + \|\hat{\ell}_0 - \ell_0\|_{P,2}\Big) \leq \delta_N N^{-1/2}$.
    \end{itemize}
\end{itemize}
\end{assumption}
Under Assumption \ref{assumption::plm}, Remark 2 holds (cf. Theorem 4.1 in \citet{Chernozhukov2018dml}). To apply Theorem 1 using a calibrated propensity score estimator, Assumption 4 has to be satisfied. To this end, we introduce the following Assumption \ref{assumption::plm_calibration_rate}.
\begin{assumption}[Calibration rate and complexity]\label{assumption::plm_calibration_rate}
Let $\tilde{m}(X)$ be an estimator of $\tilde{m}_0(X):=\E[D|\hat{m}(X)]$. We assume
\begin{itemize}
    \item[(i)] The following convergence rates hold with $P$-probability no less than $1 - \Delta_N$,
    \begin{align*}
        \|\tilde{m}(X) - \tilde{m}_0(X)\|_{P,2}\lesssim \varepsilon_N,
    \end{align*}
    such that
    \begin{align*}
        \varepsilon_N \cdot \Big(\varepsilon_N + \|\hat{\ell}_0 - \ell_0\|_{P,2}\Big) \le \delta_N N^{-1/2}.
    \end{align*}
    \item[(ii)] Let $\tilde{m}(\cdot) \in \mathcal{M}$, such that the covering numbers obey
    \begin{align*}
        \sup_{Q} N(\epsilon, \mathcal{M}, L_2(Q))\le C\epsilon^{-1}.
    \end{align*}
\end{itemize}
\end{assumption}
It is worth noting that this calibration assumption does not necessarily require $D$ to be binary.

\begin{theorem}\label{theorem::plm}
    Under Assumptions \ref{assumption::plm} and \ref{assumption::plm_calibration_rate}(i) Remark 3 is valid. If additionally Assumption \ref{assumption::plm_calibration_rate}(ii) is satisfied, Theorem 1 holds.
\end{theorem}
The proof of Theorem \ref{theorem::plm} is similar to the proof of Theorem 2 and is therefore left out. It just needs an additional complexity argument to verify Assumption 4 (ii) based on Assumption \ref{assumption::plm_calibration_rate}(ii).

==> paper/sections/theory/additional_proofs.tex <==
It holds
\begin{align*}
    \ &\|\hat{m}(X) - m_0(X)\|_{P,2}^2\\
    =\ & \mathbb{E}\left[\big(m_0(X) - \mathbb{E}[m_0(X)|\hat{m}(X)] + \mathbb{E}[m_0(X)|\hat{m}(X)] - \hat{m}(X)\big)^2\right]\\
    =\ & \mathbb{E}\left[\mathbb{E}\left[\big(m_0(X) - \mathbb{E}[m_0(X)|\hat{m}(X)] + \mathbb{E}[m_0(X)|\hat{m}(X)] - \hat{m}(X)\big)^2|\hat{m}(X)\right]\right]\\
    =\ & \mathbb{E}\left[\textrm{Var}\big(m_0(X)|\hat{m}(X)\big)\right] + \|\mathbb{E}[m_0(X)|\hat{m}(X)] - \hat{m}(X)\|_{P,2}^2\\
    & +2\mathbb{E}\left[\big(\mathbb{E}[m_0(X)|\hat{m}(X)] - \hat{m}(X)\big)\underbrace{\mathbb{E}\left[\big(m_0(X) - \mathbb{E}[m_0(X)|\hat{m}(X)]\big)|\hat{m}(X)\right]}_{=0}\right]
\end{align*}
such that
\begin{align*}
    \|\hat{m}(X) - m_0(X)\|_{P,2} &= \left(\mathbb{E}\left[\textrm{Var}\big(m_0(X)|\hat{m}(X)\big)\right] + \|\mathbb{E}[m_0(X)|\hat{m}(X)] - \hat{m}(X)\|_{P,2}^2 \right)^{1/2}.
\end{align*}

\begin{customproof}[Lemma 1]
Under Assumption 1 we can decompose the root-mean-squared-error as follows
\begin{align*}
    \|\tilde{m}(X) - m_0(X)\|_{P,2}
    &\le \underbrace{\|\tilde{m}(X) - \mathbb{E}[D|\hat{m}(X)]\|_{P,2}}_{\le \tilde{\varepsilon}_N} + \|\mathbb{E}[D|\hat{m}(X)] - m_0(X)\|_{P,2}\\
    &\le \left(\mathbb{E}\left[\V\big(m_0(X)|\hat{m}(X)\big)\right]\right)^{1/2} + \tilde{\varepsilon}_N
\end{align*}
due to 
\begin{align*}
    \|\mathbb{E}[D|\hat{m}(X)] - m_0(X)\|^2_{P,2} &= \|\mathbb{E}[m_0(X)|\hat{m}(X)] - m_0(X)\|^2_{P,2}\\ 
    &= \mathbb{E}\left[\mathbb{E}\left[\big(m_0(X) - \mathbb{E}[m_0(X)|\hat{m}(X)] \big)^2\right]|\hat{m}(X)\right]\\
    & =\mathbb{E}\left[\V\big(m_0(X)|\hat{m}(X)\big)\right].
\end{align*}
Here, we used that
\begin{align*}
    \sigma(\hat{m}(X))\subseteq \sigma(X),
\end{align*}
such that
\begin{align*}
    \mathbb{E}[m_0(X)|\hat{m}(X)] = \mathbb{E}[\mathbb{E}[D|X]|\hat{m}(X)] = \mathbb{E}[D|\hat{m}(X)].
\end{align*}
\end{customproof}

==> paper/sections/theory/dml_proof.tex <==
For any $k\in\{1,\dots,K\}$, we use the following empirical process notation
$$\G_{n,k}\left[\phi\left(W\right)\right]=\frac{1}{\sqrt{n}}\sum_{i\in I_k}\left(\phi(W_i)-\int\phi(w)dP_N\right)$$
for any $P_N$-integrable function $\phi$ on $\mathcal{W}$.

\begin{customproof}[Theorem \ref{main-theorem::dml_asympt_dist_calibration}]
    This proof adjusts the proof of Theorem 3.1 in \citet{Chernozhukov2018dml}.
    Upon inspecting the Step 1 (DML2 case) of the proof of Theorem 3.1 in \citet{Chernozhukov2018dml}, it is worth noting that the only terms which are affected by the calibration are
    \begin{align*}
        \tilde{R}_{N,1}:&= \frac{1}{K}\sum_{k=1}^K\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W_i;(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\\
        \tilde{R}_{N,2}:&= \frac{1}{K}\sum_{k=1}^K\E_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \frac{1}{N}\sum_{i=1}^N\psi\left(W_i;\theta_0,(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)
    \end{align*}
    as the other terms do not depend on the calibrated element $\tilde{\eta}^{(2)}_{0,k}$. 
    % The next steps show analogous formulations of (A.5) and (A.6) from \citet{Chernozhukov2018dml} for $|\tilde{R}_{N,1}|$ and $|\tilde{R}_{N,2}|$. 
    First, we focus on the term $\tilde{R}_{N,2}$. Following Step 3 of the proof of Theorem 3.1, we obtain by triangle inequality
    \begin{align*}
        \left|\E_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \frac{1}{n}\sum_{i\in I_k}\psi\left(W_i;\theta_0,(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right| \le \frac{\mathcal{I}_{3,k} + \mathcal{I}_{4,k}}{\sqrt{n}},
    \end{align*}
    where
    \begin{align*}
        \mathcal{I}_{3,k} &:= \left|\G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \G_{n,k}\left[\psi\left(W;\theta_0,(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\right|\\
        \mathcal{I}_{4,k} &:= \sqrt{n}\left|\E\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\big|(W_i)_{i\in I_k^c}\right] - \E\left[\psi\left(W;\theta_0,(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\right|.
    \end{align*}
    Due to Assumption \ref{main-assumption::dml} it holds $(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k}) \in \widetilde{\mathcal{T}}_N$ with probability $\ge 1-\Delta_N$.
    Define $\mathcal{E}_N$ as the event that $(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k}) \in \widetilde{\mathcal{T}}_N$ for all $k\in [K]$. Therefore, $P(\mathcal{E}_N)\ge 1-K\Delta_N$.
    Consequently, the whole argument of \citet{Chernozhukov2018dml} is still valid which implies
    \begin{align*}
        \mathcal{I}_{4,k} = O_{P_N}(\sqrt{n}(\lambda_N + \lambda'_N)).
    \end{align*}
    Next, due to the triangle inequality
    \begin{align*}
        \mathcal{I}_{3,k}&\le \left|\G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\right|\\
        & \quad + \left|\G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right] - \G_{n,k}\left[\psi\left(W;\theta_0,(\eta^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\right|\\
        &=:\ \mathcal{I}_{3,k}^{(1)} + \mathcal{I}_{3,k}^{(2)},
    \end{align*}
    where 
    $\mathcal{I}_{3,k}^{(2)} = O_{P_N}(r'_N)$ by Assumption \ref{main-assumption::dml}.2,  see \citet{Chernozhukov2018dml}.
    To bound $\mathcal{I}_{3,k}^{(1)}$, we rely on classical empirical process theory. Since conditionally on $(W_i)_{i\in I_k^c}$ the $\hat{\eta}^{(1)}_{0,k}$ is non-stochastic, remark that 
    \begin{align*}
        &\E\left[\mathcal{I}_{3,k}^{(1)}| (W_i)_{i\in I_k^c}\right] \\
        = &\E\Bigg[\left|\G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \tilde{\eta}^{(2)}_{0,k})\right)\right] - \G_{n,k}\left[\psi\left(W;\theta_0,(\hat{\eta}^{(1)}_{0,k}, \eta^{(2)}_{0,k})\right)\right]\right|\Bigg| (W_i)_{i\in I_k^c}\Bigg] \\
        \le &\sup_{\eta^{(1)} \in \widetilde{\mathcal{T}}^{(1)}_N}\E\Bigg[\sup_{\eta^{(2)}: (\eta^{(1)}, \eta^{(2)})\in\widetilde{\mathcal{T}}_N}\bigg|\G_{n,k}\left[\psi\left(W;\theta_0,(\eta^{(1)}, \eta^{(2)})\right)\right] \\
        &\quad - \G_{n,k}\left[\psi\left(W;\theta_0,(\eta^{(1)}, \eta^{(2)}_{0,k})\right)\right]\bigg|\Bigg| (W_i)_{i\in I_k^c}\Bigg] \\
        \le & \sup_{\eta^{(1)} \in \tilde{\mathcal{T}_N}^{(1)}}\E\Big[\sup_{f\in\F_2(\eta^{(1)})}|\G_{n,k}(f)| \Big| (W_i)_{i\in I_k^c}\Big]\\
        \le &\sup_{\eta^{(1)} \in \tilde{\mathcal{T}_N}^{(1)}} \E[\sup_{f\in\F_2(\eta^{(1)})}|\G_{n,k}(f)|]\\
        = &\sup_{\eta^{(1)} \in \tilde{\mathcal{T}_N}^{(1)}}\|\G_{n,k}\|_{\F_2(\eta^{(1)})}
    \end{align*}
    where $\mathcal{F}_2$ is defined in Assumption \ref{main-assumption::dml_calibration_complexity}.
    Let $\eta^{(1)}$ be a any element of $\widetilde{\mathcal{T}}_N^{(1)}$. Relying on Theorem 5.2 of \citet{10.1214/14-AOS1230}, it holds
    \begin{align*}
        \E\left[\|\G_{n,k}\|_{\F_2(\eta^{(1)})}\right]&\lesssim J\left(\delta_n, \F_2(\eta^{(1)}), F_2(\eta^{(1)})\right) \|F_2(\eta^{(1)})\|_{P,2}\\
        &\quad + \frac{\|M\|_{P,2}J^2\left(\delta_n, \F_2(\eta^{(1)}), F_2(\eta^{(1)})\right)}{\delta_n^2 \sqrt{n}} 
    \end{align*}
    with $\delta_n = \sigma_n / \|F_2(\eta^{(1)})\|_{P,2}$, $M = \max_{1\le i\le n} F_{2}(\eta^{(1)})(W_i)$, where $\sup_{f\in\F_2(\eta^{(1)})} \E[f^2] \le \sigma^2_n \le \|F_2(\eta^{(1)})\|_{P,2}^2$. Under Assumption \ref{main-assumption::dml_calibration_complexity}(i) and using $\|M\|_{P,q} \le n^{1/q}  \|F_2(\eta^{(1)})\|_{P,q}$ this implies
    \begin{align*}\E\left[\|\G_{n,k}\|_{\F_2(\eta^{(1)})}\right]&\lesssim u_n \|F_2(\eta^{(1)})\|_{P,2} + n^{1/q - 1/2} V_n u_n^2\frac{\|F_2(\eta^{(1)})\|_{P,2} ^2}{\sigma^{2}_n}.
    \end{align*}
    This enables the use of Theorem 5.1 of \citet{10.1214/14-AOS1230} with $t=\log(n)$ such that for any fixed $\eta^{(1)} \in \widetilde{\mathcal{T}}_N^{(1)}$
    \begin{align*}
        \|\G_{n,k}\|_{\F_2(\eta^{(1)})} &\le (1 + \alpha) \E\left[\|\G_{n,k}\|_{\F_2(\eta^{(1)})}\right]\\
        & \quad + C(q) \left[\left(\sigma_n + \frac{\|M\|_{P,q}}{\sqrt{n}}\right)\sqrt{\log(n)} + \frac{\|M\|_{P,2}\log(n)}{\alpha\sqrt{n}}\right]\\
        &\lesssim (1 + \alpha) \left(u_n \|F_2(\eta^{(1)})\|_{P,2} + n^{1/q - 1/2} V_n u_n^2\frac{\|F_2(\eta^{(1)})\|_{P,2} ^2}{\sigma_n^{2}} \right)\\
        & \quad + C(q) \left((\sigma_n + n^{1/q-1/2}V_n) \sqrt{\log(n)} +  n^{1/q-1/2}V_n\frac{\log(n)}{\alpha}\right)
    \end{align*}
    with probability $> 1-\log(n)^{-q/2}$ for all $\alpha > 0$ and $C(q)>0$ is a constant only depending on $q$. Consequently
    \begin{align*}
        \|\G_{n,k}\|_{\F_2(\eta^{(1)})}
        &\lesssim u_n \|F_2(\eta^{(1)})\|_{P,2} + \sigma_n \sqrt{\log(n)} \\
        & \quad +  n^{1/q-1/2}V_n \left(u_n^2\frac{\|F_2(\eta^{(1)})\|_{P,2} ^2}{\sigma_n^{2}}\vee\log(n)\right)\\
        &\le \tilde{r}_N
    \end{align*}
    with probability $> 1-c\log(n)^{-1}$, where $\tilde{r}_N$ does not depend on $\eta^{(1)}$ due to growth condition \ref{main-assumption::dml_calibration_complexity} (iii). Hence, by Lemma 6.1 in \citet{Chernozhukov2018dml}
    \begin{align*}
        \mathcal{I}_{3,k}^{(1)} = O_{P_N}(\tilde{r}_N).
    \end{align*}
    This implies that
    \begin{align*}
        |\tilde{R}_{N,2}| = O_{P_N}(N^{-1/2} (r'_N + \tilde{r}_N) + \lambda_N + \lambda'_N)
    \end{align*}
    Next, we show $|\tilde{R}_{N,1}|= |\hat{J}_0 - J_0|=O_{P_N}\left(N^{-1/2}+r_N+ \tilde{r}^a_N\right)$.
    As in \citet{Chernozhukov2018dml} is suffices to show that for any $k\in [K]$,
    \begin{align*}
        &\left|\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W;(\eta^{(1)}_{0},\eta^{(2)}_{0,k})\right)\right]\right|\\
        =& O_{P_N}(N^{-1/2} + r_N + \tilde{r}_N).
    \end{align*}
    It holds
    \begin{align*}
    &\left|\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W;(\eta^{(1)}_{0},\eta^{(2)}_{0,k})\right)\right]\right|\\
    \le& \left|\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\\
    &\quad + \left|\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right] - \E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)|(W_i)_{i\in I_k^c}\right]\right|\\
    &\quad + \left|\E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)|(W_i)_{i\in I_k^c}\right] - \E\left[\psi^a\left(W;(\eta^{(1)}_{0},\eta^{(2)}_{0,k})\right)\right]\right|\\
     =& \mathcal{I}_{1,k}^{(1)} + \mathcal{I}_{1,k}^{(2)} + \mathcal{I}_{2,k},
    \end{align*}
    where $\mathcal{I}_{1,k}^{(2)} = O_{P_N}(N^{-1/2})$ and $\mathcal{I}_{2,k} = O_{P_N}(r_N)$ by the same terms as in Step 2 of the proof of Theorem 3.1 in \citet{Chernozhukov2018dml}.
    Next, we show $\mathcal{I}_{1,k}^{(1)} = O_{P_N}(r_N + \tilde{r}_N)$.
    \begin{align*}
        \mathcal{I}_{1,k}^{(1)}
        &= \left|\E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\\
        &\le \left|\G_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \G_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\\
        &\quad + \left|\E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|
    \end{align*}
    At first, remark
    \begin{align*}
        &\left|\E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\\
        \le &\left|\E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right)\right] - \E\left[\psi^a\left(W;(\eta^{(1)}_{0},\eta^{(2)}_{0})\right)\right]\right|\\
        & + \left|\E\left[\psi^a\left(W;(\eta^{(1)}_{0},\eta^{(2)}_{0})\right)\right] - \E\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\\
        &\lesssim r_N + \tilde{r}^a_N
    \end{align*}
    by Assumption \ref{main-assumption::dml_calibration_complexity} (ii). Further, with the same argument as above
    \begin{align*}
        &\E\left[\left|\G_{n,k}\left[\psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\tilde{\eta}^{(2)}_{0,k})\right) - \psi^a\left(W;(\hat{\eta}^{(1)}_{0,k},\eta^{(2)}_{0})\right)\right]\right|\Bigg|(W_i)_{i\in I_k^c}\right]\\
        \le &\sup_{\eta^{(1)} \in \tilde{\mathcal{T}_N}^{(1)}}\|\G_{n,k}\|_{\F^a_2(\eta^{(1)})}
    \end{align*}
    with
    \begin{align*}
        \F^a_2(\eta^{(1)}):&=\left\{\psi^a\left(\cdot; (\eta^{(1)}, \eta^{(2)})\right)- \psi^a\left(\cdot; (\eta^{(1)}, \eta^{(2)}_0)\right)\big|(\eta^{(1)}, \eta^{(2)}) \in \widetilde{\mathcal{T}}_N\right\}.
    \end{align*}
    Following the same arguments as above, combined with Assumption \ref{main-assumption::dml_calibration_complexity} (ii), we obtain
    \begin{align*}
        \|\G_{n,k}\|_{\F^a_2(\eta^{(1)})}
        &\lesssim u_{n,a} \|F^a_2(\eta^{(1)})\|_{P,2} + \sigma_{n,a} \sqrt{\log(n)} \\
        & \quad +  n^{1/q-1/2}V_{n,a} \left(u_{n,a}^2\frac{\|F^a_2(\eta^{(1)})\|_{P,2} ^2}{\sigma_{n,a}^{2}}\vee\log(n)\right)\\
        &\le \tilde{r}^a_N.
    \end{align*}
    Again, by Lemma 6.1 in \citet{Chernozhukov2018dml}
    \begin{align*}
        \mathcal{I}_{1,k}^{(1)} = O_{P_N}(r_N + \tilde{r}^a_N)
    \end{align*}
    and therefore
    \begin{align*}
        |\tilde{R}_{N,1}|=O_{P_N}\left(N^{-1/2}+r_N+ \tilde{r}^a_N\right).
    \end{align*}
\end{customproof}



\begin{customproof}[Theorem \ref{main-theorem::irm}]
    The first part is an application of Theorem 5.1 \citet{Chernozhukov2018dml} with nuisance realization set $\widetilde{\mathcal{T}}_N$.\\
    The second part follows by verifying Assumption \ref{main-assumption::dml_calibration_complexity}. At first remark that Assumption \ref{main-assumption::dml_calibration_complexity}(ii) holds since $\psi^a(W;\eta) = -1$ for all $\eta \in T$. Further, it holds
    \begin{align*}
        &\mathbb{E} \left[ \left( \psi \left(W;\theta_0, (\eta^{(1)},\eta^{(2)})\right) - \psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)}_0)\right) \right)^2 \right]^{1/2}\\
        = &\left\| \psi \left(W;\theta_0, (\eta^{(1)},\eta^{(2)})\right) - \psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)}_0)\right)\right\|_{P,2}\\
        \le &\mathcal{I}_1 + \mathcal{I}_2
    \end{align*}
    with
    \begin{align*}
        \mathcal{I}_1 &:= \left\|\left(\tilde{m}(X)^{-1} - m_0(X)^{-1}\right)D(Y-g(1,X)) \right\|_{P,2}\\
        \mathcal{I}_2 &:= \left\|\left((1-\tilde{m}(X))^{-1} - (1-m_0(X))^{-1}\right)(1-D)(Y-g(0,X)) \right\|_{P,2}.
    \end{align*}
    Remark that $\epsilon \le m_0(X)\le 1-\epsilon$ and $\epsilon \le \tilde{m}(X)\le 1-\epsilon$, such that
    \begin{align*}
        \mathcal{I}_1 
        &\le \epsilon^{-2} \left\|(m_0(X) - \tilde{m}(X)) D (Y-g(1,X))\right\|_{P,2}\\
        &\le \epsilon^{-2} \left\|(m_0(X) - \tilde{m}(X)) (g_0(1,X) + U -g(1,X))\right\|_{P,2}\\
        &\le \epsilon^{-2} \left\|(m_0(X) - \tilde{m}(X)) (g_0(1,X)-g(1,X))\right\|_{P,2} + \epsilon^{-2}\left\|(m_0(X) - \tilde{m}(X))U\right\|_{P,2}\\
        &\lesssim\left\|m_0(X) - \tilde{m}(X)\right\|_{P,2} 
    \end{align*}
    since $\E[U^2|X]\le C$ and $\|g - g_0\|_{P,\infty}\le C$. 
    With a analogous argument it holds
    \begin{align*}
        \mathcal{I}_2 
        &\lesssim\left\|m_0(X) - \tilde{m}(X)\right\|_{P,2}.
    \end{align*}
    This implies
    \begin{align*}
    &\sup_{f\in\mathcal{F}_2(\eta^{(1)})}\|f\|^2_{P,2}\\
        \le &\sup_{(\eta^{(1)},\eta^{(2)})\in \widetilde{\mathcal{T}}_N} \mathbb{E} \left[ \left( \psi \left(W;\theta_0, (\eta^{(1)},\eta^{(2)})\right) - \psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)}_0)\right) \right)^2 \right] \\
        \le &\ C \left\|m_0(X) - \tilde{m}(X)\right\|^2_{P,2}\\
        \lesssim &\ \epsilon_N^2.
    \end{align*}
    
    Further, remark that using the same argument as above
    \begin{align*}
        &\left|\psi \left(W;\theta_0, (\eta^{(1)},\eta^{(2)})\right) - \psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)}_0)\right)\right|\\
        \lesssim & | m_0(X) - \tilde{m}(X)| |D(Y-g(1,X)) + (1-D)(Y-g(0,X))|\\
        \le & L(W) |m_0(X) - \tilde{m}(X)|
    \end{align*}
    where 
    \begin{align*}
        \sup_{\eta^{(1)}\in\widetilde{\mathcal{T}}_N^{(1)}}\|L(W)\|_{P,q} \lesssim \|U\|_{P,q} + \sup_{\eta^{(1)}\in\widetilde{\mathcal{T}}_N^{(1)}}\|g_0(D,X) - g(D,X)\|_{P,q} \lesssim 1.
    \end{align*}
    Applying Lemma O.1 from \cite{belloni2018uniformly} implies
    \begin{align*}
         &\log \sup_Q N(\epsilon \|L(W)\|_{Q,2}, \mathcal{F}_2 (\eta^{(1)}), \|\cdot\|_{Q,2})\\
         \le &\log \sup_Q N(\epsilon, \mathcal{M}, \|\cdot\|_{Q,2}) \\
         \le & C\epsilon^{-1}
    \end{align*}
    by Assumption \ref{main-assumption::irm_calibration_rate} (ii) , where we can use $1$ as an envelope for $\mathcal{M}$. According to the discussion of Assumption \ref{main-assumption::dml_calibration_complexity}, it holds
    \begin{align*}
        u_n\lesssim \sigma_n^{1/2} \|F_2(\eta^{(1)})\|_{P,2}^{-1/2}.
    \end{align*}
    Further, 
    \begin{align*}
        \|F_2(\eta^{(1)})\|_{P,q} 
        &\le \bigg\| \sup_{\eta^{(2)}\in\widetilde{\mathcal{T}}_N^{(2)}}\Big(\psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)})\right) - \psi\left(W;\theta_0, (\eta^{(1)},\eta^{(2)}_0)\right)\Big)\bigg\|_{P,q}\\
        &=\bigg\| L(W)\sup_{\eta^{(2)}\in\widetilde{\mathcal{T}}_N^{(2)}} |\eta^{(2)}(X) - \eta^{(2)}_0(X)|\bigg\|_{P,q}\lesssim 1.
    \end{align*}
Choose $\sigma_n=\epsilon_N \vee \log^{1/2}(n)n^{1/q-1/2}$, such that
    \begin{align*}
         \sup_{f\in \F_2(\eta^{(1)})}\|f\|_{P,2}^2 &\le \sigma_n^2\le \|F_2(\eta^{(1)})\|_{P,2}^2
    \end{align*}
for each $\eta^{(1)}$ and $n$ large enough.
Consequently,
\begin{align*}
    &\sigma_n^{1/2}  \sup_{\eta^{(1)}\in \widetilde{\mathcal{T}}_N^{(1)}} \|F_2(\eta^{(1)})\|_{P,2}^{1/2} + \sigma_n \sqrt{\log(n)}\\
    &\quad +  n^{1/q-1/2}V_n \left(\frac{ \sup_{\eta^{(1)}\in \widetilde{\mathcal{T}}_N^{(1)}} \|F_2(\eta^{(1)})\|_{P,2}}{\sigma_n^{}}\vee\log(n)\right)\\
    &\le C\sigma_n  + \sigma_n \sqrt{\log(n)} +  Cn^{1/q-1/2} \left(\sigma_n^{-1}\vee\log(n)\right)=o(1).
\end{align*}
\end{customproof}

==> paper/sections/theory/isotonic_regression.tex <==
\subsection{Theoretical Guarantees for Isotonic Regression}\label{ch:isotonic_theory}
We consider an estimated propensity score $\hat{m}(\cdot)$ based on a separate sample such that $\hat{m}(\cdot)$ can be considered a fixed function. Let $U:=\hat{m}(X)$ and define the pseudo sample as $Z:=(D,U)$, where $(Z_i)_{i=1}^n$ are iid copies of $Z$.
\todo[inline]{
Of course it would be perfect if results hold for the cross-fitted version of $\hat{m}(\cdot)$ but this messes up our iid assumption.
}

\subsection{Convergence of Isotonic Regression}
Consider the following assumptions
\begin{assumption} \label{assumption::monotonicity}
    The regression function 
    \begin{align*}
    \tilde{m}_0(u):= \E[D|U = u]
    \end{align*}
    is monotone.
\end{assumption}
\todo[inline]{
I think this is the main property we should investigate. Remark that this is much weaker than monotonicity with respect to all values of $X$, but could be identical if $\hat{m}(X)$ is bijective
}
Define $\tilde{m}$ as the estimator obtained by isotonic regression on the sample $(Z_i)_{i=1}^n$.
\begin{theorem}[Convergence of Isotonic Regression]\label{theorem::convergence_isotonic_regression}
Under Assumption \ref{assumption::monotonicity} it holds
\begin{align*}
    \|\tilde{m}(U) - \tilde{m}_0(U)\|_{P,2} = O_P(n^{-2/3}).
\end{align*}
\end{theorem}
\todo[inline]{
If necessary we can also rates on $$\|\tilde{m}(U) - \tilde{m}_0(U)\|_{\infty}=o_P(n^{-{2/9}}\log(n)^c)$$
under smoothness conditions (see \citet{mammen2007additive}).
}
\begin{customproof}[Theorem \ref{theorem::convergence_isotonic_regression}]
    At first, remark that the bracketing entropy of the function class 
    \begin{align*}
        \F_{\text{monotone}}:=\{f:\R \mapsto [0,1]|\text{f monotone}\}
    \end{align*}
    is of order $1/\epsilon$. It holds
    \begin{align*}
        \log N_{[\ ]}(\epsilon, \F_{\text{monotone}}, \|\cdot\|_{P,q})\le C \frac{1}{\epsilon}
    \end{align*}
    for all $q\ge 1$ and $C$ depends on $q$ only (Theorem 2.7.5 \citet{vaart2023empirical}).
    The result follows from similar steps as in the proof of Lemma 3 in \citet{mammen2007additive}.
    Define 
    \begin{align*}
       \varepsilon_i := D_i - \E[D_i|U_i = u]
    \end{align*}
    with $|\varepsilon_i|\le 1$. Using Theorem 9.1 from \citet{geer2000empirical} one obtains
    \todo[]{In detail?}
    \begin{align*}
        \|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P_n,2} = O_P(n^{-2/3}).
    \end{align*}
    Afterwards, since $\F_{\text{monotone}}$ is uniformly bounded, it follows from Lemma 5.15 \citet{geer2000empirical}
    \begin{align*}
        &P\left(\left|\|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P_n,2} - \|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P,2}\right|\ge \log(n)^{-1} n^{-1/3}\right)\\
        \le\ & 2\exp\left(- \frac{\log(n)^{-2}n^{1/3}}{8(\log(n)^{-1}n^{-1/3} + 1)}\right)
    \end{align*}
    This implies 
    \begin{align*}
        P\left(\|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P,2} \ge  \log(n)^{-1} n^{-1/3}\right) = o(1).
    \end{align*}
    Again, applying Lemma 5.15 \citet{geer2000empirical} implies
    \begin{align*}
        &P\left(\left|\|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P_n,2} - \|\tilde{m}(U) - \tilde{m}_0(U)\|^2_{P,2}\right|\ge n^{-2/3}\right)\\
        \le\ & 2\exp\left(- \frac{n^{-1/3}}{8(n^{-2/3} + \log(n)^{-1} n^{-1/3})}\right) + o(1)
    \end{align*}
    such that
    \begin{align*}
        \|\tilde{m}(U) - \tilde{m}_0(U)\|_{P,2} = O_P(n^{-2/3}).
    \end{align*}
\end{customproof}

==> paper/tables/table_ipw.tex <==
\vspace{-1em}
\begin{table}[h!]
\begin{center}
    \captionsetup{justification=centering}
    \begin{footnotesize}
    \begin{singlespace}
\caption{IPW Results 2}
 \label{tab:results_ipw}
        \scalebox{0.8}{
\centering
\begin{tabular}{llccccccccc}
\toprule
DGP & Method & \multicolumn{3}{c}{m = Logit} & \multicolumn{3}{c}{m = Random Forest} & \multicolumn{3}{c}{m = LGBM} \\
 &  & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. \\
\midrule
\multirow{12}{*}{1} & Alg-1-Clipped & 0.08 & 0.11 & 0.11 & 0.18 & 0.19 & 0.06 & 0.94 & 0.98 & 0.31 \\
& Alg-1-Uncalib & 0.10 & 0.16 & 0.16 & 1.09e+06 & 1.09e+07 & 1.09e+07 & 1.57 & 1.77 & 0.83 \\
& Alg-2-nested-cf-IVAP & 0.10 & 0.12 & 0.09 & 0.14 & 0.15 & 0.07 & 0.17 & 0.19 & 0.08\\
& Alg-2-nested-cf-Iso & 0.20 & 0.25 & 0.19 & 0.13 & 0.17 & 0.16 & 0.13 & \textbf{0.16} & 0.16\\
& Alg-2-nested-cf-Platt & 0.10 & 0.17 & 0.17 & 0.14 & 0.15 & 0.06 & 0.22 & 0.23 & 0.06 \\
& Alg-3-cf-IVAP & 0.11 & 0.13 & 0.07 & 0.14 & 0.16 & 0.07 & 0.17 & 0.18 & 0.07\\
& Alg-3-cf-Iso & 0.09 & 0.11 & 0.07 & 0.13 & 0.15 & 0.06 & 0.15 & 0.17 & 0.06 \\
& Alg-3-cf-Platt & 0.13 & 0.14 & 0.06 & 0.35 & 0.36 & 0.05 & 0.31 & 0.31 & 0.05 \\
& Alg-4-single-split-IVAP & 0.11 & 0.12 & 0.07 & 0.31 & 0.31 & 0.03 & 0.33 & 0.33 & 0.04\\
& Alg-4-single-split-Iso & 0.13 & 0.18 & 0.16 & 0.30 & 0.30 & 0.03 & 0.32 & 0.32 & 0.04 \\
& Alg-4-single-split-Platt & 0.10 & 0.12 & 0.09 & 0.16 & 0.17 & 0.06 & 0.23 & 0.24 & 0.06 \\
& Alg-5-full-sample-IVAP & 0.08 & 0.10 & 0.08 & 0.12 & \textbf{0.14} & 0.07 & 0.14 & \textbf{0.16} & 0.07 \\
& Alg-5-full-sample-Iso & 0.07 & \textbf{0.09} & 0.08 & 0.12 & \textbf{0.14} & 0.06 & 0.14 & \textbf{0.16} & 0.07 \\
& Alg-5-full-sample-Platt & 0.09 & 0.11 & 0.10 & 0.14 & 0.16 & 0.06 & 0.22 & 0.22 & 0.05 \\
\hline
\multirow{12}{*}{2} & Alg-1-Clipped & 0.09 & 0.12 & 0.11 & 4.45 & 4.59 & 1.11 & 2.67 & 2.74 & 0.61\\
& Alg-1-Uncalib & 0.09 & 0.12 & 0.11 & 1.17e+10 & 1.37e+10 & 7.23e+09 & 2.86 & 2.98 & 0.81 \\
& Alg-2-nested-cf-IVAP & 0.21 & 0.26 & 0.26 & 0.28 & 0.33 & 0.26 & 0.29 & 0.33 & 0.25 \\
& Alg-2-nested-cf-Iso & 0.60 & 0.81 & 0.66 & 0.47 & 0.61 & 0.61 & 0.48 & 0.64 & 0.62 \\
& Alg-2-nested-cf-Platt & 0.20 & 0.25 & 0.25 & 0.29 & 0.34 & 0.24 & 0.29 & 0.34 & 0.23 \\
& Alg-3-cf-IVAP & 0.10 & 0.12 & 0.12 & 0.21 & 0.24 & 0.12 & 0.20 & 0.23 & 0.11\\
& Alg-3-cf-Iso & 0.09 & \textbf{0.11} & 0.11 & 0.21 & 0.24 & 0.11 & 0.20 & 0.23 & 0.11 \\
& Alg-3-cf-Platt & 0.13 & 0.16 & 0.11 & 0.44 & 0.45 & 0.11 & 0.50 & 0.51 & 0.10 \\
& Alg-4-single-split-IVAP & 0.11 & 0.14 & 0.14 & 0.96 & 0.97 & 0.14 & 0.90 & 0.91 & 0.11 \\
& Alg-4-single-split-Iso & 0.61 & 0.77 & 0.53 & 0.95 & 0.96 & 0.14 & 0.87 & 0.88 & 0.11\\
& Alg-4-single-split-Platt & 0.10 & 0.12 & 0.11 & 0.26 & 0.28 & 0.12 & 0.27 & 0.29 & 0.11 \\
& Alg-5-full-sample-IVAP & 0.09 & \textbf{0.11} & 0.11 & 0.20 & \textbf{0.22} & 0.11 & 0.18 & \textbf{0.20} & 0.11 \\
& Alg-5-full-sample-Iso & 0.09 & \textbf{0.11} & 0.11 & 0.20 & 0.23 & 0.10 & 0.18 & \textbf{0.20} & 0.10\\
& Alg-5-full-sample-Platt & 0.10 & 0.12 & 0.11 & 0.27 & 0.29 & 0.10 & 0.27 & 0.29 & 0.10 \\
\hline
\multirow{12}{*}{3} & Alg-1-Clipped & 0.06 & \textbf{0.08} & 0.08 & 0.54 & 0.58 & 0.21 & 2.00 & 2.02 & 0.31\\
& Alg-1-Uncalib & 0.06 & \textbf{0.08} & 0.08 & 3.07e+08 & 8.49e+08 & 7.91e+08 & 2.05 & 2.07 & 0.34 \\
& Alg-2-nested-cf-IVAP & 0.12 & 0.15 & 0.14 & 0.36 & 0.38 & 0.11 & 0.46 & 0.48 & 0.11\\
& Alg-2-nested-cf-Iso & 0.94 & 1.03 & 0.41 & 0.26 & \textbf{0.32} & 0.31 & 0.27 & \textbf{0.34} & 0.34 \\
& Alg-2-nested-cf-Platt & 0.11 & 0.14 & 0.14 & 0.40 & 0.42 & 0.10 & 0.53 & 0.54 & 0.10 \\
& Alg-3-cf-IVAP & 0.07 & \textbf{0.08} & 0.08 & 0.32 & 0.33 & 0.08 & 0.38 & 0.38 & 0.07 \\
& Alg-3-cf-Iso & 0.07 & 0.09 & 0.08 & 0.36 & 0.37 & 0.07 & 0.42 & 0.42 & 0.07\\
& Alg-3-cf-Platt & 0.12 & 0.14 & 0.07 & 0.87 & 0.87 & 0.08 & 0.82 & 0.82 & 0.08 \\
& Alg-4-single-split-IVAP & 0.07 & 0.09 & 0.09 & 1.13 & 1.13 & 0.07 & 1.03 & 1.03 & 0.08 \\
& Alg-4-single-split-Iso & 0.73 & 0.80 & 0.34 & 1.13 & 1.13 & 0.07 & 1.03 & 1.03 & 0.08 \\
& Alg-4-single-split-Platt & 0.08 & 0.09 & 0.08 & 0.44 & 0.45 & 0.08 & 0.57 & 0.57 & 0.08 \\
& Alg-5-full-sample-IVAP & 0.06 & \textbf{0.08} & 0.08 & 0.35 & 0.36 & 0.07 & 0.40 & 0.41 & 0.07 \\
& Alg-5-full-sample-Iso & 0.06 & \textbf{0.08} & 0.08 & 0.37 & 0.37 & 0.07 & 0.42 & 0.43 & 0.07\\
& Alg-5-full-sample-Platt & 0.07 & 0.09 & 0.08 & 0.42 & 0.43 & 0.07 & 0.52 & 0.53 & 0.07\\
\hline
\multirow{12}{*}{4} & Alg-1-Clipped & 0.13 & 0.15 & 0.06 & 0.54 & 0.55 & 0.13 & 6.14 & 6.17 & 0.52 \\
& Alg-1-Uncalib & 0.13 & 0.15 & 0.06 & 4.64e+08 & 6.89e+08 & 5.11e+08 & 8.37 & 8.45 & 1.21 \\
& Alg-2-nested-cf-IVAP & 0.10 & 0.13 & 0.11 & 0.12 & 0.15 & 0.11 & 0.11 & 0.14 & 0.11\\
& Alg-2-nested-cf-Iso & 0.21 & 0.24 & 0.13 & 0.19 & 0.23 & 0.13 & 0.25 & 0.29 & 0.15 \\
& Alg-2-nested-cf-Platt & 0.13 & 0.16 & 0.11 & 0.15 & 0.18 & 0.11 & 0.15 & 0.18 & 0.12 \\
& Alg-3-cf-IVAP & 0.05 & \textbf{0.05} & 0.05 & 0.06 & \textbf{0.08} & 0.05 & 0.06 & \textbf{0.07} & 0.06 \\
& Alg-3-cf-Iso & 0.05 & 0.06 & 0.05 & 0.09 & 0.10 & 0.05 & 0.07 & 0.09 & 0.06 \\
& Alg-3-cf-Platt & 0.07 & 0.09 & 0.06 & 0.13 & 0.16 & 0.10 & 0.18 & 0.23 & 0.16 \\
& Alg-4-single-split-IVAP & 0.05 & 0.06 & 0.06 & 1.40 & 1.41 & 0.09 & 1.43 & 1.43 & 0.07 \\
& Alg-4-single-split-Iso & 0.07 & 0.09 & 0.07 & 0.88 & 0.98 & 0.43 & 0.96 & 1.02 & 0.37 \\
& Alg-4-single-split-Platt & 0.10 & 0.12 & 0.06 & 0.12 & 0.13 & 0.06 & 0.12 & 0.13 & 0.05 \\
& Alg-5-full-sample-IVAP & 0.06 & 0.08 & 0.06 & 0.10 & 0.11 & 0.05 & 0.09 & 0.10 & 0.06 \\
& Alg-5-full-sample-Iso & 0.07 & 0.08 & 0.05 & 0.11 & 0.12 & 0.05 & 0.10 & 0.11 & 0.06 \\
& Alg-5-full-sample-Platt & 0.09 & 0.11 & 0.06 & 0.12 & 0.13 & 0.06 & 0.12 & 0.13 & 0.06 \\
\bottomrule
\end{tabular}
}
\caption*{\scriptsize DGP 1: n = 2000, p = 20, R2\_d = 0.5; DGP 2: n = 2000, p = 3, overlap = 0.5; \\ DGP 3: n = 2000, p = 4; DGP 4: n = 4000, p = 20, share treated = 0.1; g = LGBM, \\ lowest RMSEs per DGP and propensity learner are highlighted}
    \end{singlespace}
    \end{footnotesize}
\end{center}
\end{table}
\vspace{-3em}


==> paper/tables/table_irm.tex <==
\begin{table}[h!]
\begin{center}
    \begin{footnotesize}
    \begin{singlespace}
    \captionsetup{justification=centering}
\caption{IRM Results}
 \label{tab:results_irm}
        \scalebox{0.8}{
\centering
\begin{tabular}{llccccccccc}
\toprule
DGP & Method & \multicolumn{3}{c}{m = Logit} & \multicolumn{3}{c}{m = Random Forest} & \multicolumn{3}{c}{m = LGBM} \\
 &  & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. \\
\midrule
\multirow{12}{*}{1} & Alg-1-Clipped & 0.07 & 0.10 & 0.10 & 0.06 & 0.08 & 0.07 & 0.22 & 0.27 & 0.24 \\
 & Alg-1-Uncalib & 0.08 & 0.13 & 0.13 & 1.85e+06 & 1.85e+07 & 1.84e+07 & 0.48 & 0.60 & 0.54 \\
 & Alg-2-nested-cf-IVAP & 0.07 & 0.09 & 0.08 & 0.06 & \textbf{0.08} & 0.07 & 0.07 & \textbf{0.08} & 0.08 \\
 & Alg-2-nested-cf-Iso & 0.12 & 0.15 & 0.14 & 0.10 & 0.12 & 0.12 & 0.10 & 0.12 & 0.12 \\
 & Alg-2-nested-cf-Platt & 0.08 & 0.14 & 0.14 & 0.06 & \textbf{0.08} & 0.07 & 0.07 & \textbf{0.08} & 0.07 \\
 & Alg-3-cf-IVAP & 0.06 & 0.08 & 0.07 & 0.06 & \textbf{0.08} & 0.08 & 0.07 & \textbf{0.08} & 0.07 \\
 & Alg-3-cf-Iso & 0.06 & 0.08 & 0.07 & 0.06 & \textbf{0.08} & 0.08 & 0.06 & \textbf{0.08} & 0.07 \\
 & Alg-3-cf-Platt & 0.06 & \textbf{0.07} & 0.07 & 0.07 & 0.08 & 0.06 & 0.07 & \textbf{0.08} & 0.07 \\
 & Alg-4-single-split-IVAP & 0.06 & 0.08 & 0.07 & 0.07 & \textbf{0.08} & 0.06 & 0.07 & 0.09 & 0.06 \\
 & Alg-4-single-split-Iso & 0.10 & 0.13 & 0.12 & 0.07 & \textbf{0.08} & 0.06 & 0.07 & 0.09 & 0.06 \\
 & Alg-4-single-split-Platt & 0.07 & 0.08 & 0.08 & 0.06 & \textbf{0.08} & 0.07 & 0.07 & \textbf{0.08} & 0.07 \\
 & Alg-5-full-sample-IVAP & 0.07 & 0.08 & 0.08 & 0.07 & 0.09 & 0.08 & 0.07 & \textbf{0.08} & 0.08 \\
 & Alg-5-full-sample-Iso & 0.06 & 0.08 & 0.08 & 0.06 & \textbf{0.08} & 0.07 & 0.07 & \textbf{0.08} & 0.08 \\
 & Alg-5-full-sample-Platt & 0.07 & 0.09 & 0.09 & 0.06 & \textbf{0.08} & 0.07 & 0.07 & \textbf{0.08} & 0.07 \\
\hline
\multirow{12}{*}{2} & Alg-1-Clipped & 0.09 & \textbf{0.11} & 0.11 & 0.31 & 0.39 & 0.39 & 0.20 & 0.26 & 0.26 \\
 & Alg-1-Uncalib & 0.09 & \textbf{0.11} & 0.11 & 2.22e+09 & 2.89e+09 & 2.86e+09 & 0.24 & 0.32 & 0.32 \\
 & Alg-2-nested-cf-IVAP & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & 0.12 & 0.12 \\
 & Alg-2-nested-cf-Iso & 0.18 & 0.23 & 0.22 & 0.16 & 0.22 & 0.22 & 0.19 & 0.24 & 0.24 \\
 & Alg-2-nested-cf-Platt & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
 & Alg-3-cf-IVAP & 0.09 & \textbf{0.11} & 0.11 & 0.10 & 0.12 & 0.12 & 0.10 & 0.12 & 0.12 \\
 & Alg-3-cf-Iso & 0.09 & \textbf{0.11} & 0.11 & 0.09 & 0.12 & 0.12 & 0.10 & 0.12 & 0.12 \\
 & Alg-3-cf-Platt & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
 & Alg-4-single-split-IVAP & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
 & Alg-4-single-split-Iso & 0.15 & 0.20 & 0.20 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
 & Alg-4-single-split-Platt & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
 & Alg-5-full-sample-IVAP & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & 0.12 & 0.12 \\
 & Alg-5-full-sample-Iso & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & 0.12 & 0.12 \\
 & Alg-5-full-sample-Platt & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.11 \\
\hline
\multirow{12}{*}{3} & Alg-1-Clipped & 0.05 & 0.07 & 0.07 & 0.08 & 0.10 & 0.10 & 0.11 & 0.13 & 0.13 \\
 & Alg-1-Uncalib & 0.05 & 0.07 & 0.07 & 9.97e+07 & 2.74e+08 & 2.73e+08 & 0.11 & 0.14 & 0.14 \\
 & Alg-2-nested-cf-IVAP & 0.05 & 0.07 & 0.07 & 0.05 & \textbf{0.07} & 0.06 & 0.05 & \textbf{0.07} & 0.07 \\
 & Alg-2-nested-cf-Iso & 0.10 & 0.13 & 0.12 & 0.08 & 0.10 & 0.10 & 0.10 & 0.13 & 0.13 \\
 & Alg-2-nested-cf-Platt & 0.05 & 0.07 & 0.07 & 0.05 & \textbf{0.07} & 0.06 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-3-cf-IVAP & 0.05 & 0.07 & 0.06 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.07 \\
 & Alg-3-cf-Iso & 0.05 & 0.07 & 0.07 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-3-cf-Platt & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.07} & 0.06 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-4-single-split-IVAP & 0.05 & 0.07 & 0.07 & 0.05 & \textbf{0.07} & 0.06 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-4-single-split-Iso & 0.10 & 0.12 & 0.11 & 0.05 & \textbf{0.07} & 0.06 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-4-single-split-Platt & 0.05 & 0.07 & 0.06 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.06 \\
 & Alg-5-full-sample-IVAP & 0.05 & 0.07 & 0.07 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.07 \\
 & Alg-5-full-sample-Iso & 0.05 & 0.07 & 0.07 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.07 \\
 & Alg-5-full-sample-Platt & 0.05 & 0.07 & 0.07 & 0.06 & \textbf{0.07} & 0.07 & 0.05 & \textbf{0.07} & 0.06 \\
\hline
\multirow{12}{*}{4} & Alg-1-Clipped & 0.04 & 0.06 & 0.06 & 0.07 & 0.09 & 0.09 & 0.17 & 0.21 & 0.20 \\
 & Alg-1-Uncalib & 0.04 & 0.06 & 0.06 & 1.74e+08 & 2.70e+08 & 2.68e+08 & 0.36 & 0.46 & 0.43 \\
 & Alg-2-nested-cf-IVAP & 0.04 & \textbf{0.05} & 0.05 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-2-nested-cf-Iso & 0.05 & 0.07 & 0.07 & 0.05 & 0.07 & 0.07 & 0.06 & 0.07 & 0.07 \\
 & Alg-2-nested-cf-Platt & 0.04 & 0.06 & 0.05 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-3-cf-IVAP & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-3-cf-Iso & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-3-cf-Platt & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-4-single-split-IVAP & 0.04 & 0.06 & 0.06 & 0.04 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-4-single-split-Iso & 0.05 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-4-single-split-Platt & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-5-full-sample-IVAP & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-5-full-sample-Iso & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.06 \\
 & Alg-5-full-sample-Platt & 0.04 & 0.06 & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.04 & \textbf{0.06} & 0.05 \\
\bottomrule
\end{tabular}
}
\caption*{\scriptsize DGP 1: n = 2000, p = 20, R2\_d = 0.5; DGP 2: n = 2000, p = 3, overlap = 0.5; \\ DGP 3: n = 2000, p = 4; DGP 4: n = 4000, p = 20, share treated = 0.1; g = LGBM, \\ lowest RMSEs per DGP and propensity learner are highlighted}
    \end{singlespace}
    \end{footnotesize}
\end{center}
\end{table}
\vspace{-2em}


==> paper/tables/table_plr.tex <==
\begin{table}[h!]
\begin{center}
    \begin{footnotesize}
    \begin{singlespace}
    \captionsetup{justification=centering}
    \caption{PLR Results}
    \label{tab:results_plr}
        \scalebox{0.8}{
\centering
\begin{tabular}{llccccccccc}
\toprule
DGP & Method & \multicolumn{3}{c}{m = Logit} & \multicolumn{3}{c}{m = Random Forest} & \multicolumn{3}{c}{m = LGBM} \\
 &  & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. & MAE & RMSE & Std. dev. \\
\midrule
\multirow{12}{*}{1} & Alg-1-Clipped & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-1-Uncalib & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-2-nested-cf-IVAP & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-2-nested-cf-Iso & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-2-nested-cf-Platt & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-3-cf-IVAP & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-3-cf-Iso & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & 0.07 & 0.07 \\
 & Alg-3-cf-Platt & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & 0.07 & 0.07 \\
 & Alg-4-single-split-IVAP & 0.05 & \textbf{0.06} & 0.06 & 0.14 & 0.18 & 0.18 & 0.12 & 0.15 & 0.15 \\
 & Alg-4-single-split-Iso & 0.05 & \textbf{0.06} & 0.06 & 0.15 & 0.20 & 0.20 & 0.13 & 0.16 & 0.16 \\
 & Alg-4-single-split-Platt & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-5-full-sample-IVAP & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
 & Alg-5-full-sample-Iso & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & 0.07 & 0.07 \\
 & Alg-5-full-sample-Platt & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 & 0.05 & \textbf{0.06} & 0.06 \\
\hline
\multirow{12}{*}{2} & Alg-1-Clipped & 0.09 & \textbf{0.11} & 0.10 & 0.12 & 0.14 & 0.10 & 0.10 & 0.11 & 0.10 \\
 & Alg-1-Uncalib & 0.09 & \textbf{0.11} & 0.10 & 0.12 & 0.14 & 0.10 & 0.10 & 0.11 & 0.10 \\
 & Alg-2-nested-cf-IVAP & 0.09 & \textbf{0.11} & 0.10 & 0.10 & 0.12 & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-2-nested-cf-Iso & 0.09 & \textbf{0.11} & 0.10 & 0.10 & 0.12 & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-2-nested-cf-Platt & 0.09 & \textbf{0.11} & 0.10 & 0.10 & 0.12 & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-3-cf-IVAP & 0.09 & \textbf{0.11} & 0.10 & 0.10 & 0.12 & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-3-cf-Iso & 0.09 & \textbf{0.11} & 0.11 & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.10} & 0.10 \\
 & Alg-3-cf-Platt & 0.09 & \textbf{0.11} & 0.10 & 0.11 & 0.13 & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-4-single-split-IVAP & 0.09 & \textbf{0.11} & 0.10 & 0.23 & 0.26 & 0.14 & 0.13 & 0.16 & 0.12 \\
 & Alg-4-single-split-Iso & 0.09 & \textbf{0.11} & 0.10 & 0.24 & 0.27 & 0.15 & 0.13 & 0.16 & 0.12 \\
 & Alg-4-single-split-Platt & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.11} & 0.10 & 0.09 & 0.11 & 0.10 \\
 & Alg-5-full-sample-IVAP & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.10} & 0.10 \\
 & Alg-5-full-sample-Iso & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.10} & 0.10 \\
 & Alg-5-full-sample-Platt & 0.09 & \textbf{0.11} & 0.10 & 0.09 & \textbf{0.11} & 0.10 & 0.09 & 0.11 & 0.10 \\
\hline
\multirow{12}{*}{3} & Alg-1-Clipped & 0.06 & \textbf{0.08} & 0.08 & 0.06 & \textbf{0.07} & 0.07 & 0.08 & 0.10 & 0.07 \\
 & Alg-1-Uncalib & 0.06 & \textbf{0.08} & 0.08 & 0.06 & \textbf{0.07} & 0.07 & 0.08 & 0.10 & 0.07 \\
 & Alg-2-nested-cf-IVAP & 0.06 & \textbf{0.08} & 0.08 & 0.07 & 0.09 & 0.07 & 0.09 & 0.11 & 0.07 \\
 & Alg-2-nested-cf-Iso & 0.06 & \textbf{0.08} & 0.08 & 0.07 & 0.09 & 0.07 & 0.09 & 0.11 & 0.07 \\
 & Alg-2-nested-cf-Platt & 0.06 & \textbf{0.08} & 0.08 & 0.07 & 0.08 & 0.07 & 0.09 & 0.11 & 0.07 \\
 & Alg-3-cf-IVAP & 0.06 & \textbf{0.08} & 0.08 & 0.06 & 0.08 & 0.07 & 0.06 & 0.08 & 0.07 \\
 & Alg-3-cf-Iso & 0.07 & 0.09 & 0.08 & 0.06 & 0.08 & 0.08 & 0.06 & 0.08 & 0.08 \\
 & Alg-3-cf-Platt & 0.07 & \textbf{0.08} & 0.08 & 0.10 & 0.12 & 0.08 & 0.07 & 0.09 & 0.08 \\
 & Alg-4-single-split-IVAP & 0.06 & \textbf{0.08} & 0.08 & 1.01 & 1.02 & 0.16 & 0.43 & 0.44 & 0.11 \\
 & Alg-4-single-split-Iso & 0.06 & \textbf{0.08} & 0.08 & 1.10 & 1.11 & 0.18 & 0.46 & 0.47 & 0.12 \\
 & Alg-4-single-split-Platt & 0.06 & \textbf{0.08} & 0.08 & 0.06 & 0.08 & 0.08 & 0.08 & 0.09 & 0.07 \\
 & Alg-5-full-sample-IVAP & 0.06 & \textbf{0.08} & 0.08 & 0.06 & 0.08 & 0.07 & 0.06 & \textbf{0.08} & 0.07 \\
 & Alg-5-full-sample-Iso & 0.07 & 0.09 & 0.08 & 0.06 & \textbf{0.07} & 0.07 & 0.06 & \textbf{0.07} & 0.07 \\
 & Alg-5-full-sample-Platt & 0.06 & \textbf{0.08} & 0.08 & 0.06 & 0.08 & 0.08 & 0.06 & \textbf{0.07} & 0.07 \\
\hline
\multirow{12}{*}{4} & Alg-1-Clipped & 0.08 & \textbf{0.09} & 0.06 & 0.05 & \textbf{0.06} & 0.05 & 0.05 & \textbf{0.06} & 0.05 \\
 & Alg-1-Uncalib & 0.08 & \textbf{0.09} & 0.06 & 0.05 & \textbf{0.06} & 0.05 & 0.05 & \textbf{0.06} & 0.05 \\
 & Alg-2-nested-cf-IVAP & 0.08 & \textbf{0.09} & 0.05 & 0.07 & 0.09 & 0.05 & 0.07 & 0.09 & 0.05 \\
 & Alg-2-nested-cf-Iso & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.07 & 0.09 & 0.05 \\
 & Alg-2-nested-cf-Platt & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.07 & 0.09 & 0.05 \\
 & Alg-3-cf-IVAP & 0.07 & \textbf{0.09} & 0.06 & 0.07 & 0.08 & 0.05 & 0.07 & 0.09 & 0.05 \\
 & Alg-3-cf-Iso & 0.08 & 0.10 & 0.06 & 0.08 & 0.09 & 0.05 & 0.08 & 0.10 & 0.05 \\
 & Alg-3-cf-Platt & 0.08 & \textbf{0.09} & 0.05 & 0.07 & 0.09 & 0.05 & 0.08 & 0.09 & 0.06 \\
 & Alg-4-single-split-IVAP & 0.08 & 0.10 & 0.06 & 0.56 & 0.59 & 0.19 & 0.56 & 0.58 & 0.14 \\ & Alg-4-single-split-Iso & 0.08 & \textbf{0.09} & 0.06 & 0.26 & 0.31 & 0.17 & 0.26 & 0.30 & 0.16 \\
 & Alg-4-single-split-Platt & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.08 & 0.09 & 0.05 \\
 & Alg-5-full-sample-IVAP & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.08 & 0.09 & 0.05 \\
 & Alg-5-full-sample-Iso & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.08 & 0.09 & 0.05 \\
 & Alg-5-full-sample-Platt & 0.08 & \textbf{0.09} & 0.06 & 0.07 & 0.09 & 0.05 & 0.08 & 0.09 & 0.05 \\
\bottomrule
\end{tabular}
}
\caption*{\scriptsize DGP 1: n = 2000, p = 20, R2\_d = 0.5; DGP 2: n = 2000, p = 3, overlap = 0.5; \\ DGP 3: n = 2000, p = 4; DGP 4: n = 4000, p = 20, share treated = 0.1; g = LGBM, \\ lowest RMSEs per DGP and propensity learner are highlighted}
    \end{singlespace}
    \end{footnotesize}
\end{center}
\end{table}
\vspace{-2em}


==> paper/tables/weightit_comp.tex <==
\begin{table}[h!]
\begin{center}
\captionsetup{justification=centering}
\caption{Comparison under covariate balance}
\label{tab:weightit_comp}
    \begin{footnotesize}
    \begin{singlespace}
        \scalebox{0.7}{
\centering
\begin{tabular}{lllrrrrrrrr}
\toprule
Method &  & m & Coverage & CI Length & Norm $D=1$ & Norm $D=0$ & RMSE & Std. dev. & MAE \\
\midrule
Alg-3-cf & isotonic & Logit & 0.960 & 0.413 & 0.996 & 0.987 & 0.098 & 0.097 & 0.077 \\
Alg-3-cf & isotonic & RF & 0.960 & 0.389 & 0.997 & 0.994 & 0.096 & 0.094 & 0.075 \\
Alg-3-cf & platt & Logit & 0.960 & 0.388 & 1.003 & 0.984 & 0.094 & 0.093 & 0.075 \\
Alg-3-cf & platt & RF & 0.940 & 0.358 & 0.984 & 0.961 & 0.092 & 0.091 & 0.072 \\
Alg-5-full-sample & isotonic & Logit & 0.970 & 0.404 & 0.999 & 0.998 & 0.097 & 0.095 & 0.077 \\
Alg-5-full-sample & isotonic & RF & 0.940 & 0.386 & 1.000 & 1.000 & 0.095 & 0.094 & 0.075 \\
Alg-5-full-sample & platt & Logit & 0.960 & 0.397 & 1.003 & 0.996 & 0.094 & 0.093 & 0.075 \\
Alg-5-full-sample & platt & RF & 0.950 & 0.373 & 0.998 & 0.988 & 0.094 & 0.093 & 0.074 \\
Cbps & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.074 \\
Ebal & weighted & \- & 0.950 & 0.376 & 1.000 & 1.000 & 0.094 & 0.093 & 0.074 \\
Glm & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.075 \\
Ipt & weighted & Logit & 0.950 & 0.371 & 1.000 & 1.000 & 0.094 & 0.093 & 0.075 \\
Optweight & weighted & \- & 0.960 & 0.376 & 1.000 & 1.000 & 0.093 & 0.092 & 0.074 \\
\bottomrule
\end{tabular}
}
\caption*{\scriptsize DGP 2: n = 2000, p = 3, overlap = 0.5, Clip = 1e-12, g = Linear}
    \end{singlespace}
    \end{footnotesize}
    		\end{center}
\end{table}

